A Simple Approach to Continual Learning by Transferring Skill Parameters

In order to be effective general purpose machines in real world environments, robots not only will need to adapt their existing manipulation skills to new circumstances, they will need to acquire entirely new skills on-the-fly. A great promise of continual learning is to endow robots with this ability, by using their accumulated knowledge and experience from prior skills. We take a fresh look at this problem, by considering a setting in which the robot is limited to storing that knowledge and experience only in the form of learned skill policies. We show that storing skill policies, careful pre-training, and appropriately choosing when to transfer those skill policies is sufficient to build a continual learner in the context of robotic manipulation. We analyze which conditions are needed to transfer skills in the challenging Meta-World simulation benchmark. Using this analysis, we introduce a pair-wise metric relating skills that allows us to predict the effectiveness of skill transfer between tasks, and use it to reduce the problem of continual learning to curriculum selection. Given an appropriate curriculum, we show how to continually acquire robotic manipulation skills without forgetting, and using far fewer samples than needed to train them from scratch.

==> 06_towards_skill_policy.tex <==
In this section we introduce a novel policy model which allows us to rapidly acquire new skills by mixing parameters and behavior from an entire skill library at once, rather than by reusing only one skill at a time.
We share promising results towards using this policy model class for continual learning.
As this policy model infers online which skill behaviors and parameters to use for acquiring a new skill, it can be interpreted as a form of active curriculum selection for continual learning~\cite{foglino2019curriculum}.


\subsection{Policy Model and Pre-Training Procedure}
In Section~\ref{sec:skill_curriculums}, we showed that we could use an offline cost metric calculation on the task space to solve for an efficient continual learning curriculum.
This has the obvious downside of requiring exhaustive evaluation of all skill-skill pairs in the task space.
Prior work has shown that, for large enough task spaces, it is possible to build an inference model to predict the skill-skill transfer cost by pre-training an inference model using data from a representative sample of the task space~\cite{sinapov2015learning}.
However, we believe the ideal algorithm for this setting would learn to infer skill-skill transfer cost online, rather than requiring offline pre-training.

\begin{figure}[h]
    \centering
    \includegraphics[height=2in, width=\textwidth]{figures/mcp_diagram_freehand.png}
    \caption{Diagram of a policy model class for active skill curriculum selection operating on two tasks, $\tau$ and $\tau'$.
    This model class allows RL agents to reuse both parameters and behavior from all skills in a library during fine-tuning, and uses RL supervision actively select which skills with which to explore and which skills' parameters to update.
    Note that arrows are not shown from $s_{\tau'}$ to $\pi_i$ for visual clarity.
    }
    \label{fig:mcp_diagram}
\end{figure}

In order to perform this inference online, we would need to collect data on the effectiveness the all skills in the skill library online during training, and dynamically select which skills are most beneficial for the current target task.
Previous works~\cite{finn2019online} have described how to achieve this with implicit inference on neural network parameters.
We recall our observations from this work that, for RL for manipulation skills, it is reusing skill behavior which is most important for continual learning performance.
``How can we infer online which skill \textit{behaviors} are most beneficial for learning the current task?'' If we can somehow execute all skill policies from the skill library at once as the base policy during fine-tuning, on-policy RL thankfully provides us with the answer to the inference question, in the form of the policy gradient estimator.

We propose a policy model architecture for rapid fine-tuning of skill behaviors based on a probabilistic product-of-experts model.
Our policy model class is similar to that proposed by~\citeauthor{peng2019mcp} for use for adaptation in imitation learning and~\citeauthor{tseng2021toward} for meta-RL.
The policy model (Figure~\ref{fig:mcp_diagram}) is composed of a library of skill policies $\pi_{i = 1 \ldots k}(a|s)$\footnote{\ie each skill policy is a Gaussian distribution parameterized by observation-conditioned mean and variance functions} and a learned observation-conditioned mixing function $w_\tau$ for each target task $\tau$.
Note that unlike in previous sections, the number of skill policies in the library is independent of the number of tasks.
The mixing functions share the skill library networks, and mix them by computing a weighted product of their Gaussian distributions, where the weights are the output of the learned observation-conditioned mixing function for that task.

\begin{align}
  \pi_{\tau}(a|s) &= \frac {1} {Z(s)} \prod_{i \le k} \pi_i(a|s)^{w^{\tau}_i(s)} \\
    \quad\text{where}\quad\pi_i &= \mathcal{N}(\mu_i(s), \sigma_i(s))
\end{align}

\paragraph{Pre-training} During pre-training, we select a small subset of the task space $\mathcal{T}_{pretrain} \subset \mathcal{T}$ with which to initialize our skill library, and jointly train the independent mixing functions, and shared skill library, for all pre-train tasks $\tau_{pretrain} \in \mathcal{T}_{pretrain}$\footnote{We find that distilling single-task policies for the pre-train tasks using behavioral cloning is effective, but this step may also be performed with RL}.
Note that this joint training through the mixing functions is especially important: it forces the algorithm to learn skill policies which can be effectively mixed by the task-specific mixing functions while also solving the tasks, \ie it forces the policy class to learn to decompose the task policies into independent skills.
Our work in Section~\ref{sec:skill_curriculums} suggests that the best tasks to use for pre-training are the most difficult ones.

\paragraph{Adaptation} To adapt the skill library to a new task, we  initialize a new task-specific mixing function $w^\tau$ for that task, and use on-policy fine-tuning to select its weights.
We keep the skill policies frozen, so that they do not forget their pre-trained parameters, but new, unfrozen skill library policies may be initialized and learned at this time, to expand the library capacity.
The policy gradient loss measures the overall effectiveness of the skill mixing policy's behavior, and adjusts the relative weights of the skill in the library to maximize return on the new task.

\subsection{Early Results for Continual Learning}
\begin{figure}[h]
    \centering
    \frame{\includegraphics[width=0.45\columnwidth,valign=c]{figures/arm_failure.png}}
    \frame{\includegraphics[width=0.45\columnwidth,valign=c]{figures/arm_success.png}}
    \caption{Examples of successful and failed policy executions for adapting to the \texttt{window-open} task.
    \textbf{Left:} The skill mixing policy reaches to the window and pushes, but chooses the wrong side from which to push.
  \textbf{Right:} The skill mixing policy successfully opens the window.}
    \label{fig:mcp_rollouts}
\end{figure}

Figure~\ref{fig:mcp_performance} shows for using this policy class, pre-training, and adaptation procedure for adaptation within Meta-World MT10 (Figure~\ref{fig:metaworld_envs}).
In this experiment, the pre-train tasks are the 7 MT10 tasks not listed in the legend.
We find that this skill mixing policy class is very effective as a prior for adaptation, partially-solving two out of three test tasks in just $250,000$ environment steps.
All prior policies start training with equal or higher average returns than training from scratch.
The \texttt{drawer-close} environment is solved on the first optimization epoch.

\begin{figure}[h]
    \centering
    \includegraphics[height=2in]{figures/skill_mixing_performance_2.pdf}
    \caption{Skill mixing policy performance during fine-tuning, as measured with average discounted return.
    The skill mixing policies fine-tune very quickly to high-return policies for all 3 target tasks.
  Despite this, some policies fail to achieve full success on the task due to inadequate exploration.}
    \label{fig:mcp_performance}
\end{figure}

The task this fine-tuning procedure does not solve is \texttt{window-open}, which has an interesting failure mode (Figure~\ref{fig:mcp_rollouts}).
The skill mixing policy immediately learns to reach-to, then push-on the window handle.
Unfortunately, because it was pre-trained with \texttt{window-close}, the prior policy behavior pushes from the right side of the window handle towards the left (Figure~\ref{fig:mcp_rollouts}, Left).
A successful policy would push from the left side of the window handle towards the right (Figure~\ref{fig:mcp_rollouts}).
Our RL agent choose this policy because it failed to explore reaching to the left side of the window handle.
We find that a na{\"i}ve application of the policy model class from~\citeauthor{peng2019mcp} results in RL skill policies with low entropy, so though they encode excellent priors, they fail to explore.
In future work, we will consider how to retain the excellent behavior reuse properties of this model class while encouraging online exploration, and how to achieve online skill curriculum learning with structured exploration.

